Share Withholding Attack in Blockchain Mining: Technical Report

Cryptocurrency achieves distributed consensus using proof of work (PoW). Prior research in blockchain security identified financially incentivized attacks based on withholding blocks which have the attacker compromise a victim pool and pose as a PoW contributor by submitting the shares (earning credit for mining) but withholding the blocks (no actual contributions to the pool). We advance such threats to generate greater reward advantage to the attackers while undermining the other miners and introduce the share withholding attack (SWH). SWH withholds shares to increase the attacker's reward payout within the pool, in contrast to the prior threats withholding blocks, and rather builds on the block-withholding threats in order to exploit the information about the impending block submission timing, challenging the popularly established assumption that the block submission time is completely random and unknown to miners. We analyze SWH's incentive compatibility and the vulnerability scope by identifying the critical systems and environmental parameters which determine the attack's impact. Our results show that SWH in conjunction with block withholding yield unfair reward advantage at the expense of the protocol-complying victim miners and that a rational miner will selfishly launch SWH to maximize its reward profit. We inform the blockchain and cryptocurrency research of the novel SWH threat and include the potential countermeasure directions to facilitate such research and development.

==> discussion_real_world.tex <==
\subsection{Discussion About Real-World Practice}
\label{subsec:real_world_implementations}

While we take a model-based approach to enable formal analyses, %to derive implementation-independent insights, 
the model constructions are driven by the current systems implementations of blockchain; Section~\ref{sec:background} provides a high-level overview of the relevant background system components. 
Using the models and game-based analyses, our work identifies the system component which yields the vulnerabilities for SWH, the payout scheme, % uncle-block attack and share-withholding (as discussed previously, the two attacks can be launched separately or together), 
%and we identify 
%real-world blockchain systems which rewards uncle blocks and are vulnerable to uncle-block attack (which comprises of more than \$45B market cap in aggregate)
and derive that the mining pool systems using decaying payout are vulnerable to share-withholding attack (for example, the vulnerable systems comprise more than 12\% of computational power cap in Bitcoin). 
%; as discussed previously, share-withholding attack and uncle-block attack can be conducted separately or together. 

%While our work is to inform the design of the current and future blockchain systems, 
While our work introduces novel vulnerability and threat and shed negative lights on such system components, we do not recommend blindly discarding them since they serve useful purposes: uncle block rewards for increased fairness among the miners and decaying payout for pool-hopping resistance. 
Rather, we intend to inform the blockchain researchers and developers for their parameter decisions and future design constructions.
Replacement mechanisms and their incorporation to the overall blockchain system remains an open challenge for blockchain research and development. 
We also list other preliminary ideas for potential countermeasures, which we consider to be of lower overheads, to encourage research in preventing and mitigating share-withholding and uncle-block attack in Section~\ref{subsec:potential_countermeasures}. 

==> reward_analyses.tex <==
\section{Share-Withholding Attack Reward Analyses}

We incentivize share-withholding attack by increasing the expected reward. 
While Section~\ref{sec:incentive_compatibility} established the relevance and the scope of share-withholding attack (the share-withholding attack is incentivized when $f$ has a decaying reward), it did not quantify the actual reward amount, which varies across the mining pools and will heavily depend on the mining pool designs and other parameters. 
In this section, we analyze the reward in environments where the share-withholding attack is incentive compatible, i.e., the payout has a decaying reward and the attacker has some information about the block submission timing. 
We specifically analyze the case when the attacker has the full information about the block submission timing and the case when the attacker is conducting fork-after-withholding (FAW) attack on a victim pool; 
we use the analyses of the former case (which can also be useful for analyzing the attack impact in other scenarios) to build the analyses on the latter case. 
The FAW case provides a incentivized environment, as described in Section~\ref{subsec:related_bwh} where the attacker does have full control on the block submission timing (when it withholds the block and submits it later). 

\subsection{Theoretical Model: Computational Power}

As described in Section~\ref{sec:incentive_compatibility}, a payout scheme with a fixed reward is not subjected to share-withholding attack by a rational, incentive-driven attacker. 
However, a decaying-reward payout scheme does incentivize a rational attacker to withhold shares and delay their submissions. 
A popular implementation of a payoff with a decaying reward is in the form \emph{scores} where each share reward experiences exponential decay in reward values;
% (the weight of the rewards for the share); 
such scoring-based payoff is used in Slush, geometric, and double-geometric payout implementations. 
In other words, the reward value (the weight for the score) for a share follows the exponential function and decays by $e^{-cT}$ where $T$ is the time elapsed since the share submission and $c$ is some constant, 
i.e., a share submitted at time $x$ will have $e^{-c\Delta x}$ less reward value than the share submitted at time $x+\Delta x$ for any $x$ and any $\Delta x>0$. 
The reward is then distributed proportionally to the shares' contribution to the scores, e.g., 
the attacker's fraction of the block reward will be the sum aggregate of the scores of the shares submitted by the attacker divided by the total sum aggregate of all the shares' scores. 
For any miner $j$, the score for $j$, denoted by $S_j$, is the sum-aggregate of the scores of the shares submitted by $j$. 

To quantify the expected reward, in addition to using those in Section~\ref{sec:theo_model}, we introduce more variables. 
In each round, the mining pool which found the block wins the block reward (which can include new currency/coins and the transaction fee, which is a compensation to the miners processing the transaction/block separate), which amount is $B$. 
%The block reward minus the mining pool manager operating fee is $B$, 
%which is the amount that gets . 
The block reward amount in a round is actually a Bernoulli variable where it is equal to $B$ if the pool wins the round (i.e., block is found within the mining pool before the other mining pools find and broadcast a block solution) and is equal to 0 if the pool does not in the round (a block is found outside of the mining pool). 
Because, in the rounds corresponding to the latter case, the reward is zero regardless of the share submission strategies, 
we analyze the reward assuming that the mining pool finds the block in the round. 

While for block-withholding attack or FAW attack there is only one block per round (as the block marks the end of the round), the impact of share-withholding depends on the number of shares submitted in a round, 
which number corresponds to $\| \vec{s} \|$ where $\| \vec{x} \|$ is the number of elements of any vector $\vec{x}$. 
We also define $\gamma$ to be the ratio between the block difficulty and the share difficulty, i.e., $\gamma = \frac{D_{\mbox{block}}}{D_{\mbox{share}}}$ where $D_{\mbox{block}}$ is the measure for difficulty for finding a block and is inversely proportional to the solution threshold $\tau_{\mbox{block}}$ (described in Section~\ref{sec:intro}) and $D_{\mbox{share}}$ is the share difficulty and inversely proportional to $\tau_{\mbox{share}}$. 
$D_{\mbox{block}}$ is controlled by the blockchain system, e.g., Bitcoin adjusts it according to the total computational power so that a block gets mined approximately every ten minutes, 
and $D_{\mbox{share}}$ is to increase the contribution-estimation samples to lower the variance, e.g., aggregating more samples converge better to the mean by law of large numbers. 
$\gamma = \frac{D_{\mbox{block}}}{D_{\mbox{share}}}$ corresponds to the number of shares per blocks, i.e., for every block, a miner finds $\gamma$ shares on average. 

The reward distributed depends on the miner's computational power, and we normalize the following variables with respect to the total miner's computation power.
i.e., the total mining power has a power of 1. 
The attacker's computation power is $\alpha$ while the victim pool's mining power without the attacker is $\beta$. 
The attacker splits its power between honest mining and the attacking power on the victim pool for launching FAW attack; the fraction of the attacker's power for launching FAW is $\lambda$ 
Therefore the attacker's power on FAW attack is $\alpha \cdot \lambda$, and the mining power on the victim pool is $\alpha \lambda + \beta$ even though the attacker's power does not fully contribute to the pool earning reward, e.g., in the simpler case of block-withholding attack, the attacker does not submit block at all in the victim pool so the power contributing to block earnings of the pool is actually only $\beta$ (while the earning gets split by ~$\alpha \lambda + \beta$) and the expected reward for the pool is $\beta B$. 

In FAW attack, the attacker submits the withheld block on the victim pool only when another block by a third-party pool is getting propagated. 
The attacker is motivated to do so and cause a fork because the attacker does not get any reward if a third-party pool wins the block. 
$c$ denotes the probability that the attacker's block will get rewarded as opposed to the third-party pool's, and $c$ depends on the networking state and topology between the two blocks. 



The following summarizes the additional variables used for the reward analyses. 
\newline \indent \indent $B$: \indent Block reward 
\newline \indent \indent $\| \vec{s} \|$: $\; \; $ Number of share submissions in the round
\newline \indent \indent $S_j$: $\; \; $ Score for the miner $j$ for any $j$
\newline \indent \indent $\gamma$: \indent Ratio between the block difficulty and the share difficulty
\newline \indent \indent $\alpha$: \indent Attacker's computational power %, normalized by the total power of the network
 \newline \indent \indent $\beta$: \indent Computational power of the victim pool, excluding the attacker's
\newline \indent \indent $\tau$: \indent The fraction of attacker's power for FAW attack % (as opposed to main pool's power)



%Why do we choose these two particular scenarios? !!!!!!!!!!!!!!! The latter actually builds on the former case.!!!!!!!!!!!!

\subsection{Case of Attacker Having Perfect Information of Block Timing}
Suppose the attacker concentrates its power in one pool ($\lambda = 1$), which is in contrast to the requirement for block-withholding or FAW attacks, and knows when the block will get submitted ($t_B$).  %and the mining pool including the attacker finds the block and $\vec{s}$ includes the block. 
To maximize its reward, the share-withholding attacker submits all the shares right before $t_B$ or at $t_B-\epsilon$ where $\epsilon$ is small, 
so that all shares experience no decay in their reward values and have the maximum reward values of one. 

In a decaying-reward payout, if the mining pool wins the block, each share is expected to pay out $\frac{1}{\gamma}$ since $\gamma$ is the expected number of shares per block/round. %if the mining pool wins. 
%Therefore, the share at the time $T$ after its submission will decay in its reward value by exp($\gamma$) or by $\gamma e^{-\gamma T}$.  
An attacker behaving honestly will therefore have a reward of $ (\alpha + \beta) \cdot \frac{1}{\gamma} \cdot \frac{\alpha}{\alpha + \beta} \gamma = \alpha$ in expectation
where the $\alpha + \beta$ corresponds to the probability that the pool wins the block (against the other pools), and $\frac{1}{\gamma}$ and $\frac{\alpha}{\alpha + \beta} \gamma$ correspond to the reward per share and the number of shares (the total number of shares is $\gamma$ in expectation), respectively, given that the pool won the block. %distribution of the reward among the mining pool members given that the pool won. 
%$\alpha$ is also the computational power of the attacker mining honestly. 
%Therefore, the share at the time $T$ after its submission will decay in its reward value by exp($\frac{\gamma}{B}$) or by $\frac{\gamma}{B} e^{-\frac{\gamma}{B} T}$.  
%An attacker behaving honestly will therefore have a reward of $ (\alpha + \beta) \cdot \frac{B}{\gamma} \cdot \frac{\alpha}{\alpha + \beta} \gamma = \alpha B$ in expectation
%where the $\alpha + \beta$ corresponds to the probability that the pool wins the block (against the other pools), and $\frac{B}{\gamma}$ and $\frac{\alpha}{\alpha + \beta} \gamma$ correspond to the reward per share and the number of shares (the total number of shares is $\gamma$ in expectation), respectively, given that the pool won the block.% %distribution of the reward among the mining pool members given that the pool won. 
%%$\alpha$ is also the computational power of the attacker mining honestly. 
The resulting expected reward for the attacker behaving honestly is $\alpha$, which is its computational power normalized by the total mining power. 



An attacker conducting share-withholding attack, however, will maximize all of the share values by making $T\rightarrow0$ and having the score weight to be one. 
%and thus the expected reward is $(\alpha + \beta) \cdot \gamma \cdot \frac{\alpha}{\alpha + \beta} \gamma = \alpha \gamma^2 $. 
While each share's score contribution individually is $\gamma$ times greater than have the attacker behaved honestly, the final reward is distribution proportionally to the miner members' scores. 
The reward for the attacker $j$ increases by $\frac{S_j}{S_j + \sum_{i\neq j} S_i}$, 
and therefore the attacker reward is $\alpha \cdot \mbox{E}\left[\frac{S_j}{S_j + \sum_{i\neq j} S_i} \right]$ in expectation, where E[.] is the expected value. 
The reward gain of the miner $j$ launching share-withholding attack (SWH) and behaving honestly (and submitting the shares as they are found) is 
\begin{eqnarray}
\frac{R_{\mbox{swh}}}{R_{\mbox{honest}}} & = & \mbox{E}\left[\frac{S_j}{S_j + \sum_{i\neq j} S_i} \right] \nonumber \\ 
& = & \sum_{y=0}^\infty \sum_{x=0}^j \mbox{E} \left[ \left. \frac{x}{x+\sum_{i\neq j} S_i} \right\vert S_i = x, \|\vec{s}\| = y \right] \cdot \mbox{Pr}[S_j = x \; \bigg| \|\vec{s}\| = y] \cdot \mbox{Pr}[\|\vec{s}\|=y]   \nonumber \\ 
& = & \sum_{y=0}^\infty \sum_{x=0}^j \mbox{E} \left[ \left. \frac{x}{x+\sum_{i\neq j} S_i} \right\vert S_i = x, \|\vec{s}\| = y \right] \cdot {y \choose x} \left(\frac{\alpha}{\alpha+\beta} \right)^x \left(\frac{\beta}{\alpha+\beta} \right)^{y-x} \cdot \left( 1-\frac{1}{\gamma} \right)^{y-1} \frac{1}{\gamma}   \nonumber \\ 
& \geq & \sum_{y=0}^\infty \sum_{x=0}^j \frac{x}{x+\mbox{E}\left[ \sum_{i\neq j} S_i \right]} \cdot {y \choose x} \left(\frac{\alpha}{\alpha+\beta} \right)^x \left(\frac{\beta}{\alpha+\beta} \right)^{y-x} \cdot \left( 1-\frac{1}{\gamma} \right)^{j-1} \frac{1}{\gamma}   \nonumber \\ 
& = & \sum_{y=0}^\infty \sum_{x=0}^j {y \choose x} \frac{x}{x+\frac{\beta}{\alpha+\beta}} \cdot  \frac{\alpha^x \beta^{y-x}}{(\alpha + \beta)^y} \cdot \frac{(\gamma-1)^{y-1}}{\gamma^y}  \label{eqn:swh_reward_gain}  %\nonumber \\ 
\end{eqnarray} 
%\begin{eqnarray}
%\Delta R_{\mbox{swh}} = \alpha \left(\gamma^2 - 1 \right)
%\end{eqnarray} 
%An attacker conducting share-withholding attack, however, will maximize all of the share values by making $T\rightarrow0$ and have the share value be $\frac{\gamma}{B}$) and thus the expected reward is $(\alpha + \beta) \cdot \frac{\gamma}{B} \cdot \frac{\alpha}{\alpha + \beta} \gamma = \frac{\alpha \gamma^2}{ B} $. 
%The difference between launching share-withholding attack (SWH) and behaving honestly (and submitting the shares as they are found) is 
%\begin{eqnarray}
%\Delta R_{\mbox{swh}} = \alpha \left(\frac{ \gamma^2}{ B} - B \right)
%\end{eqnarray} 
where ${y \choose x}$ is $y$-choose-$x$ (${y \choose x} = \frac{y!}{x!(y-x)!}$)
and E[A$|$B] and Pr[A$|$B], respectively, are the expected value and the probability of event A given event B. 
The second equality is from the Bayes' rule (conditioned on the attacker's final score $S_j$ and the number of shares in the round $\vec{s}$), 
and the third equality is derived because $S_j$ has a binomial distribution with $y$ trials and $\frac{\alpha}{\alpha+\beta}$ probability (in each share, there is a $\frac{\alpha}{\alpha+\beta}$ chance that the share is being submitted by an attacker), given $\vec{s} = y$, 
and $\vec{s}$ has a geometric distribution with the parameter/probability of $\frac{1}{\gamma} = \frac{D_{\mbox{share}}}{D_{\mbox{block}}}$ (the last share in $\vec{s}$ is the one that is also a block). 
The inequality is due to Jensen's Inequality and that $\mbox{E}\left[\frac{S_j}{S_j + \sum_{i\neq j} S_i} \right]$ is convex with $S_j + \sum_{i\neq j} S_i$ given $S_j$. 
Finally, linear algebra yields the final equality. 
The final equality provides a lower bound on the attacker $j$'s reward gain, that is, the attacker's reward scales greater than the final equality. 
We define this gain as the lower-bound gain of conducting SWH attack over behaving honestly and denote it with $G_{lb}$, i.e., $G_{lb} \leq \frac{R_{\mbox{swh}}}{R_{\mbox{honest}}}$ and
\begin{eqnarray}
G_{lb} = \sum_{y=0}^\infty \sum_{x=0}^j {y \choose x} \frac{x}{x+\frac{\beta}{\alpha+\beta}} \cdot  \frac{\alpha^x \beta^{y-x}}{(\alpha + \beta)^y} \cdot \frac{(\gamma-1)^{y-1}}{\gamma^y}  
\end{eqnarray} 
%An attacker behaving honestly will therefore have a reward of $ (\alpha + \beta) \frac{\alpha}{\alpha + \beta} = \alpha$ 
%where the $\alpha + \beta$ corresponds to the expected reward that the pool wins the block (against the other pools) and $\frac{\alpha}{\alpha + \beta}$ corresponds to the distribution of the reward among the mining pool members given that the pool won. 
%$\alpha$ is also the computational power of the attacker mining honestly. 

We also introduce an approximate gain, $G_{\mbox{approx}} = \frac{\mbox{E}[S_j]}{\mbox{E}[S_j] + \mbox{E}[ \sum_{i\neq j} S_i]} \approx \mbox{E}\left[\frac{S_j}{S_j + \sum_{i\neq j} S_i} \right]$, i.e.,
%, from $\mbox{E}\left[\frac{S_j}{S_j + \sum_{i\neq j} S_i} \right] \approx \frac{\mbox{E}[S_j]}{\mbox{E}[S_j] + \mbox{E}[ \sum_{i\neq j} S_i]} = G_{\mbox{approx}}$, i.e., 
\begin{eqnarray}
G_{\mbox{approx}} & = & \frac{\mbox{E}[S_j]}{\mbox{E}[S_j] + \mbox{E}[ \sum_{i\neq j} S_i]} \nonumber \\
& = & \frac{\frac{\alpha}{\alpha+\beta}\gamma}{\frac{\alpha}{\alpha+\beta}\gamma + \frac{\beta}{\alpha+\beta} \gamma \frac{1}{\gamma}} \nonumber \\
& = & \frac{\alpha \gamma}{\alpha \gamma + \beta}
\end{eqnarray}
where $\mbox{E}[S_j] = \frac{\alpha}{\alpha+\beta}\gamma$ because the expected number of share for the attacker $j$ is $\frac{\alpha}{\alpha+\beta}\gamma$ and each share is weighted by one because of no decay, 
and $\mbox{E}[ \sum_{i\neq j} S_i] = \frac{\beta}{\alpha+\beta} \gamma \frac{1}{\gamma}$ because the expected number of share fore the rest of the miners excluding $j$ is $\frac{\beta}{\alpha+\beta} \gamma$ and each share's score contribution is decayed by $\frac{1}{\gamma}$ on average. 

!!!!!!!!!!!!!!!!!!!!!!!!!!!!

%An attacker conducting share-withholding attack, however, will maximize all of the share values (by making $T\rightarrow0$ and have the share value be $\gamma$) and thus the expected reward is $\frac{\alpha}{\alpha + \beta} \gamma$. 
%The difference between launching share-withholding attack (SWH) and behaving honestly (and submitting the shares as they are found) is 
%\begin{eqnarray}
%\Delta R_{\mbox{swh}} = \frac{\alpha}{\alpha + \beta} \gamma - \frac{\alpha}{\alpha + \beta} = \frac{\alpha}{\alpha + \beta} (\gamma-1)
%\end{eqnarray} 

%$\frac{\alpha \lambda}{\alpha \lambda + \beta} B$ in expectation because the expected number of shares submitted by an attacker is $\frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma$ where the fraction corresponds to the attacker's power with respect to the total power of the mining pool.
%exp($\frac{\gamma}{B}$) or by $\frac{\gamma}{B}e^{-\frac{\gamma}{B}T}$. 
%An attacker behaving honestly will therefore have a reward of $\frac{\alpha \lambda}{\alpha \lambda + \beta} B$ in expectation because the expected number of shares submitted by an attacker is $\frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma$ where the fraction corresponds to the attacker's power with respect to the total power of the mining pool. 

%An attacker conducting share-withholding attack, however, will maximize all of the share values (by making $T\rightarrow0$ and have the share value be $\frac{\gamma}{B}$) and thus the expected reward is $\frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma \cdot \frac{\gamma}{B}$. 
%The difference between launching share-withholding attack (SWH) and behaving honestly (and submitting the shares as they are found) is 
%\begin{eqnarray}
%\Delta R_{\mbox{swh}} = \frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma \frac{\gamma}{B} - \frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma = \frac{\alpha \lambda}{\alpha \lambda + \beta} \gamma \left( \frac{\gamma}{B} - 1 \right)
%\end{eqnarray} 

Therefore, the SWH attack grows with the attacker's power in the pool ($\alpha \lambda$), decreases with the rest of the mining pool's power ($\beta$), and quadratically with the block-to-share difficulty ratio ($\gamma$). 
Increasing $\gamma$ lowers the reward variance which is the motivation for joining mining pools ($\gamma=1$ is equivalent to solo mining since all shares are also blocks) but increases the networking overhead for broadcasting the shares. 




\subsection{FAW and SWH Attack Against a Victim Pool}
FAW attack provides a concrete case when the attacker submits a block at a particular time (reactive to cause a collision) and is therefore an opportune platform for share-withholding (SWH) attack. 
An FAW attacker submits the withheld block only when it discovers that there is a block getting propagated by a third-party pool. 
In addition, a share-withholding attacker coupled with FAW attack (SWH-FAW) withholds the shares and submits them right before the withheld blocks. 
We also assume the setup of FAW attack or the BWH attack where the attacker has a main pool (solo mining by the attacker itself and therefore no sharing of the reward) and the victim pool (compromised by the attacker and the object of the attacks). 

We build on the analyses of FAW attack~\cite{kwon2017}. 
The attacker's expected reward for launching FAW attack is: 
\begin{eqnarray}
R_{\mbox{faw}} = \frac{(1-\lambda)\alpha}{1-\lambda\alpha} + \left( \frac{\beta}{1-\lambda\alpha} + c \lambda \alpha \cdot \frac{1- \alpha - \beta}{1-\lambda \alpha} \right) \cdot \frac{\lambda \alpha}{\beta + \lambda \alpha}
\label{eqn:faw_reward}
\end{eqnarray}
The three terms correspond to distinct scenarios when the attacker gets a reward: the first term is the expected reward from its main pool (honest and solo mining); the second term corresponds to the case when the victim pool, excluding the attacker, finds the block; and the third term corresponds to a third-party pool finding a block and the attacker causing a fork by submitting the withheld block. 

The SWH-FAW attack affects the second and the third cases. 
When the victim pool, excluding the attacker, finds a block, the attacker risks loosing the reward for the withheld shares because the attacker did not submit them on time, e.g., the block reaches the mining pool manager before the attacker. 
We consider the worst case (for the attacker) when the attacker loses the share values. 
In such case, the expected reward becomes $\frac{\beta}{1-\lambda\alpha} \cdot 0 = 0$ where the fraction corresponds to the probability that the victim pool excluding the attacker finds a block. 

In the third case, $c \lambda \alpha \cdot \frac{1- \alpha - \beta}{1-\lambda \alpha} \cdot $

